Federated Multi-Mini-Batch: An Efficient Training Approach to Federated Learning in Non-IID Environments

Federated learning has faced performance and network communication challenges, especially in the environments where the data is not independent and identically distributed (IID) across the clients. To address the former challenge, we introduce the federated-centralized concordance property and show that the federated single-mini-batch training approach can achieve comparable performance as the corresponding centralized training in the Non-IID environments. To deal with the latter, we present the federated multi-mini-batch approach and illustrate that it can establish a trade-off between the performance and communication efficiency and outperforms federated averaging in the Non-IID settings.

==> ham10k.tex <==
To compare \textit{FedMMB} with \textit{FedAvg}, we employ the \textit{VGG16} model~\cite{vgg16} and the \textit{HAM10000} dataset~\cite{ham10000} in addition to \textit{4CFNN} and CIFAR-10. The \textit{HAM10000} is an imbalanced dataset, comprising of $10015$ dermatoscopic skin lesion images of seven classes: \textit{Melanocytic nevi}(6705), \textit{Melanoma} (1113), \textit{Benign keratosis} (1099), \textit{Basal cell carcinoma} (514), \textit{Actinic keratoses} (327), \textit{Vascular lesions} (142), and \textit{Dermatofibroma} (115)\footnote{The numbers inside parenthesis indicate the number of samples from each class}. The original resolution of the images is $600X450$ pixel but we downsampled them to $200X150$ to reduce the number of parameters in the model. \textit{VGG16} is a deep neural network model containing $13$ convlutional and $2$ fully-connected layers (\textit{TensorFlow} implementation). The model contains $\appox82$ million trainable parameters in our case. 

Regarding the \textit{HAM1000} dataset, we randomly split the dataset into the train set ($8012$ images) and the test set ($2003$ images). For the \textit{Non-IID} scenario, we partition the train set among three clients ( $3376$ sample from five classes, $2367$ samples of two classes, and $2269$ images from two classes) (Fig?). Notice that class \textit{Melanocytic nevi} is still the majority class in all clients and sample distribution is imbalanced across the clients. We refer this scenario as \textit{HAM-Non-IID}.

==> related_work.tex <==
Learning from real-world \textit{Non-IID} (heterogeneous) data is a crucial but still understudied problem. Recently, Hsieh et al. \cite{hsieh2019non} empirically studied the challenges of training on \textit{Non-IID} data by comparing the performance of several distributed learning algorithms including \textit{FedAvg}. They showed that data heterogeneity makes accurate federated learning very challenging, while the level of heterogeneity plays a major role in this problem. We demonstrate that \textit{FedSMB} can addresses this challenge by training an accurate federated neural network model even in \textit{Non-IID} environments with different levels of label heterogeneity (Section \ref{subsec:result-fed-smb}).
  
Li et al. \cite{li2019convergence} theoretically analyzed the convergence of FedAvg in \textit{Non-IID} settings and showed that \textit{FedAvg} with $E > 1$ and full batch might not converge to the optimum. Our results (Section \ref{subsec:resust-vs-fed-avg}) indicate that this is also the case for \textit{FedAvg} with $E=1$ and mini-batches. In both configurations, the clients update the global model multiple times, which affects the convergence of the model.
  
\textit{FedProx} \cite{li2020federated} re-parameterized \textit{FedAvg} and introduced a general federated optimization algorithm (with \textit{FedAvg} as its special case). The algorithm adds a proximal term to the clients' loss function to bound their impact on the divergence of the global model, making the model converge more robustly. \textit{FedMA} \cite{wang2020federated} proposed a layer-wise matching and averaging strategy that outperforms \textit{FedAvg} and \textit{FedProx} for \textit{Non-IID} data. \textit{FedMMB} takes a different approach and provides a trade-off between the performance and communication efficiency by controlling the number of local updates at the clients for a given batch size.
